Better than the Best: Gradient-based Improper Reinforcement Learning for Network Scheduling

We consider the problem of scheduling in constrained queueing networks with a view to minimizing packet delay. Modern communication systems are becoming increasingly complex, and are required to handle multiple types of traffic with widely varying characteristics such as arrival rates and service times. This, coupled with the need for rapid network deployment, render a bottom up approach of first characterizing the traffic and then devising an appropriate scheduling protocol infeasible. In contrast, we formulate a top down approach to scheduling where, given an unknown network and a set of scheduling policies, we use a policy gradient based reinforcement learning algorithm that produces a scheduler that performs better than the available atomic policies. We derive convergence results and analyze finite time performance of the algorithm. Simulation results show that the algorithm performs well even when the arrival rates are nonstationary and can stabilize the system even when the constituent policies are unstable.

==> figures/extra_capacity_improper_learning.tex <==


\tikzset{every picture/.style={line width=0.75pt}} %set default line width to 0.75pt        

\resizebox{7.00cm}{4.25cm}{


\begin{tikzpicture}[x=0.57pt,y=0.57pt,yscale=-1,xscale=1]
%uncomment if require: \path (0,441); %set diagram left start at 0, and has height of 441

%Shape: Axis 2D [id:dp7452783749628158] 
\draw [line width=2.25]  (22,380.5) -- (652.8,380.5)(85.08,6.97) -- (85.08,422) (645.8,375.5) -- (652.8,380.5) -- (645.8,385.5) (80.08,13.97) -- (85.08,6.97) -- (90.08,13.97)  ;
%Straight Lines [id:da9142352961854645] 
\draw [line width=1.5]    (85.8,22.98) -- (573.8,380.97) ;
%Straight Lines [id:da9886485978498722] 
\draw [color={rgb, 255:red, 74; green, 99; blue, 226 }  ,draw opacity=1 ][line width=2.25]    (85.08,379.4) -- (115.27,94.95) ;
\draw [shift={(115.8,89.98)}, rotate = 456.06] [fill={rgb, 255:red, 74; green, 99; blue, 226 }  ,fill opacity=1 ][line width=0.08]  [draw opacity=0] (16.07,-7.72) -- (0,0) -- (16.07,7.72) -- (10.67,0) -- cycle    ;
%Straight Lines [id:da01735236817527741] 
\draw [color={rgb, 255:red, 74; green, 99; blue, 226 }  ,draw opacity=1 ][line width=2.25]    (85.08,379.4) -- (461.82,349.37) ;
\draw [shift={(466.8,348.98)}, rotate = 535.44] [fill={rgb, 255:red, 74; green, 99; blue, 226 }  ,fill opacity=1 ][line width=0.08]  [draw opacity=0] (16.07,-7.72) -- (0,0) -- (16.07,7.72) -- (10.67,0) -- cycle    ;
%Shape: Rectangle [id:dp025384842686548836] 
\draw  [fill={rgb, 255:red, 128; green, 128; blue, 128 }  ,fill opacity=0.3 ] (85.08,89.98) -- (115.8,89.98) -- (115.8,379.4) -- (85.08,379.4) -- cycle ;
%Shape: Rectangle [id:dp5886792180583069] 
\draw  [fill={rgb, 255:red, 128; green, 128; blue, 128 }  ,fill opacity=0.3 ] (85.08,348.98) -- (466.8,348.98) -- (466.8,379.4) -- (85.08,379.4) -- cycle ;
%Shape: Right Triangle [id:dp16395811499058488] 
\draw  [fill={rgb, 255:red, 87; green, 19; blue, 254 }  ,fill opacity=0.3 ][dash pattern={on 2.53pt off 3.02pt}][line width=2.25]  (115.8,89.98) -- (466.8,348.98) -- (115.8,348.98) -- cycle ;
%Straight Lines [id:da10681329777672421] 
\draw    (48.8,145) -- (77.8,145) -- (98.8,145) ;
\draw [shift={(100.8,145)}, rotate = 180] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (12,-3) -- (0,0) -- (12,3) -- cycle    ;
%Straight Lines [id:da2568518717516832] 
\draw    (412.8,413.97) -- (412.8,366.97) ;
\draw [shift={(412.8,364.97)}, rotate = 450] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (12,-3) -- (0,0) -- (12,3) -- cycle    ;
%Straight Lines [id:da4078365096901999] 
\draw    (287.8,90.2) -- (189.45,188.55) ;
\draw [shift={(188.04,189.96)}, rotate = 315] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da6666951497559499] 
\draw    (484,198) -- (427.08,266.44) ;
\draw [shift={(425.8,267.97)}, rotate = 309.75] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;

% Text Node
\draw (628,388.4) node [anchor=north west][inner sep=0.75pt]  [font=\large]  {$\mathbf{\lambda _{1}}$};
% Text Node
\draw (48,22.4) node [anchor=north west][inner sep=0.75pt]  [font=\large]  {$\mathbf{\lambda _{2}}$};
% Text Node
\draw (4,82.4) node [anchor=north west][inner sep=0.75pt]    {$( 0,1-\epsilon )$};
% Text Node
\draw (435,388.4) node [anchor=north west][inner sep=0.75pt]    {$( 1-\epsilon ,0)$};
% Text Node
\draw (26,341.4) node [anchor=north west][inner sep=0.75pt]    {$( 0,\epsilon )$};
% Text Node
\draw (96,389.4) node [anchor=north west][inner sep=0.75pt]    {$( \epsilon ,0)$};
% Text Node
\draw (124,320) node [anchor=north west][inner sep=0.75pt]   [align=left] {\textbf{{\Large A}}};
% Text Node
\draw (121,69) node [anchor=north west][inner sep=0.75pt]   [align=left] {\textbf{{\large B}}};
% Text Node
\draw (468,335) node [anchor=north west][inner sep=0.75pt]   [align=left] {\textbf{{\large C}}};
% Text Node
\draw (13,138.4) node [anchor=north west][inner sep=0.75pt]    {$\mathbf{C_{2}}$};
% Text Node
\draw (401.8,418.37) node [anchor=north west][inner sep=0.75pt]    {$\mathbf{C_{2}}$};
% Text Node
\draw (237,46) node [anchor=north west][inner sep=0.75pt]   [align=left] {\begin{minipage}[lt]{126.871pt}\setlength\topsep{0pt}
\begin{center}
extra capacity achieved\\through \textbf{improper learning}
\end{center}

\end{minipage}};
% Text Node
\draw (472,170.4) node [anchor=north west][inner sep=0.75pt]  [font=\large]  {$\mathbf{\lambda _{1} \ +\ \lambda _{2} =1}$};


\end{tikzpicture}
% \begin{tikzpicture}[x=0.5pt,y=0.5pt,yscale=-1,xscale=1]
% %uncomment if require: \path (0,441); %set diagram left start at 0, and has height of 441

% %Shape: Axis 2D [id:dp7452783749628158] 
% \draw [line width=2.25]  (16,380.5) -- (646.8,380.5)(79.08,6.97) -- (79.08,422) (639.8,375.5) -- (646.8,380.5) -- (639.8,385.5) (74.08,13.97) -- (79.08,6.97) -- (84.08,13.97)  ;
% %Straight Lines [id:da9142352961854645] 
% \draw [line width=1.5]    (79.8,22.98) -- (567.8,380.97) ;
% %Straight Lines [id:da9886485978498722] 
% \draw [color={rgb, 255:red, 74; green, 99; blue, 226 }  ,draw opacity=1 ][line width=2.25]    (79.08,379.4) -- (109.27,94.95) ;
% \draw [shift={(109.8,89.98)}, rotate = 456.06] [fill={rgb, 255:red, 74; green, 99; blue, 226 }  ,fill opacity=1 ][line width=0.08]  [draw opacity=0] (16.07,-7.72) -- (0,0) -- (16.07,7.72) -- (10.67,0) -- cycle    ;
% %Straight Lines [id:da01735236817527741] 
% \draw [color={rgb, 255:red, 74; green, 99; blue, 226 }  ,draw opacity=1 ][line width=2.25]    (79.08,379.4) -- (455.82,349.37) ;
% \draw [shift={(460.8,348.98)}, rotate = 535.44] [fill={rgb, 255:red, 74; green, 99; blue, 226 }  ,fill opacity=1 ][line width=0.08]  [draw opacity=0] (16.07,-7.72) -- (0,0) -- (16.07,7.72) -- (10.67,0) -- cycle    ;
% %Shape: Rectangle [id:dp025384842686548836] 
% \draw  [fill={rgb, 255:red, 128; green, 128; blue, 128 }  ,fill opacity=0.3 ] (79.08,89.98) -- (109.8,89.98) -- (109.8,379.4) -- (79.08,379.4) -- cycle ;
% %Shape: Rectangle [id:dp5886792180583069] 
% \draw  [fill={rgb, 255:red, 128; green, 128; blue, 128 }  ,fill opacity=0.3 ] (79.08,348.98) -- (460.8,348.98) -- (460.8,379.4) -- (79.08,379.4) -- cycle ;
% %Shape: Right Triangle [id:dp16395811499058488] 
% \draw  [fill={rgb, 255:red, 87; green, 19; blue, 254 }  ,fill opacity=0.3 ][dash pattern={on 2.53pt off 3.02pt}][line width=2.25]  (109.8,89.98) -- (460.8,348.98) -- (109.8,348.98) -- cycle ;
% %Straight Lines [id:da10681329777672421] 
% \draw    (42.8,145) -- (71.8,145) -- (92.8,145) ;
% \draw [shift={(94.8,145)}, rotate = 180] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (12,-3) -- (0,0) -- (12,3) -- cycle    ;
% %Straight Lines [id:da2568518717516832] 
% \draw    (406.8,413.97) -- (406.8,366.97) ;
% \draw [shift={(406.8,364.97)}, rotate = 450] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (12,-3) -- (0,0) -- (12,3) -- cycle    ;
% %Straight Lines [id:da4078365096901999] 
% \draw    (281.8,90.2) -- (183.45,188.55) ;
% \draw [shift={(182.04,189.96)}, rotate = 315] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
% %Straight Lines [id:da6666951497559499] 
% \draw    (478,198) -- (421.08,266.44) ;
% \draw [shift={(419.8,267.97)}, rotate = 309.75] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;

% % Text Node
% \draw (622,388.4) node [anchor=north west][inner sep=0.75pt]  [font=\large]  {$\mathbf{\lambda _{1}}$};
% % Text Node
% \draw (48,22.4) node [anchor=north west][inner sep=0.75pt]  [font=\large]  {$\mathbf{\lambda _{2}}$};
% % Text Node
% \draw (11,82.4) node [anchor=north west][inner sep=0.75pt]    {$( 0,1-\epsilon )$};
% % Text Node
% \draw (429,385.4) node [anchor=north west][inner sep=0.75pt]    {$( 1-\epsilon ,0)$};
% % Text Node
% \draw (32,341.4) node [anchor=north west][inner sep=0.75pt]    {$( 0,\epsilon )$};
% % Text Node
% \draw (90,387.4) node [anchor=north west][inner sep=0.75pt]    {$( \epsilon ,0)$};
% % Text Node
% \draw (118,320) node [anchor=north west][inner sep=0.75pt]   [align=left] {\textbf{{\Large A}}};
% % Text Node
% \draw (115,69) node [anchor=north west][inner sep=0.75pt]   [align=left] {\textbf{{\large B}}};
% % Text Node
% \draw (462,335) node [anchor=north west][inner sep=0.75pt]   [align=left] {\textbf{{\large C}}};
% % Text Node
% \draw (18,138.4) node [anchor=north west][inner sep=0.75pt]    {$\mathbf{C_{2}}$};
% % Text Node
% \draw (395.8,416.37) node [anchor=north west][inner sep=0.75pt]    {$\mathbf{C_{2}}$};
% % Text Node
% \draw (231,49) node [anchor=north west][inner sep=0.75pt]   [align=left] {\begin{minipage}[lt]{126.871pt}\setlength\topsep{0pt}
% \begin{center}
% extra capacity achieved\\through \textbf{improper learning}
% \end{center}

% \end{minipage}};
% % Text Node
% \draw (466,170.4) node [anchor=north west][inner sep=0.75pt]  [font=\large]  {$\mathbf{\lambda _{1} \ +\ \lambda _{2} =1}$};


% \end{tikzpicture}
}

==> figures/fig_queueing_motivation.tex <==


\tikzset{every picture/.style={line width=0.75pt}} %set default line width to 0.75pt        
% SYNTAX: \resizebox{width}{height}
\resizebox{9.50cm}{3.75cm}{

\begin{tikzpicture}[x=0.5pt,y=0.5pt,yscale=-1,xscale=1]
%uncomment if require: \path (0,273); %set diagram left start at 0, and has height of 273

%Straight Lines [id:da09715700995858345] 
\draw [line width=1.5]    (81.8,155.36) -- (260.8,155.36) ;
%Straight Lines [id:da8887479227991981] 
\draw [line width=1.5]    (80.8,215.36) -- (260.8,216.36) ;
%Straight Lines [id:da6217209993953612] 
\draw    (61.8,185.36) -- (89.8,185.36) ;
\draw [shift={(91.8,185.36)}, rotate = 180] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da875509031522369] 
\draw [line width=1.5]    (260.8,155.36) -- (260.8,216.36) ;
%Straight Lines [id:da37671038244024846] 
\draw    (180,45) -- (257.8,45) ;
\draw [shift={(260.8,45)}, rotate = 180] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (8.93,-4.29) -- (0,0) -- (8.93,4.29) -- cycle    ;
\draw [shift={(177,45)}, rotate = 0] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (8.93,-4.29) -- (0,0) -- (8.93,4.29) -- cycle    ;
%Straight Lines [id:da0678614898035077] 
\draw    (122.8,225) -- (257.8,225) ;
\draw [shift={(260.8,225)}, rotate = 180] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (8.93,-4.29) -- (0,0) -- (8.93,4.29) -- cycle    ;
\draw [shift={(119.8,225)}, rotate = 0] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (8.93,-4.29) -- (0,0) -- (8.93,4.29) -- cycle    ;
%Shape: Circle [id:dp028275738414681006] 
\draw  [fill={rgb, 255:red, 155; green, 155; blue, 155 }  ,fill opacity=0.67 ] (365,142.18) .. controls (365,134) and (371.63,127.36) .. (379.82,127.36) .. controls (388,127.36) and (394.64,134) .. (394.64,142.18) .. controls (394.64,150.37) and (388,157) .. (379.82,157) .. controls (371.63,157) and (365,150.37) .. (365,142.18) -- cycle ;
%Curve Lines [id:da7202837492936005] 
\draw    (343.8,77.36) .. controls (279.45,122.9) and (302.33,173.34) .. (342.58,204.43) ;
\draw [shift={(343.8,205.36)}, rotate = 217.09] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da4678251099443136] 
\draw    (365,142.18) -- (288.45,89.5) ;
\draw [shift={(286.8,88.36)}, rotate = 394.53999999999996] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Shape: Axis 2D [id:dp8494447421977243] 
\draw [line width=1.5]  (472,195.73) -- (648.8,195.73)(489.68,64) -- (489.68,210.36) (641.8,190.73) -- (648.8,195.73) -- (641.8,200.73) (484.68,71) -- (489.68,64) -- (494.68,71)  ;
%Shape: Right Triangle [id:dp441461564376495] 
\draw  [fill={rgb, 255:red, 155; green, 155; blue, 155 }  ,fill opacity=0.25 ] (489,95) -- (610.8,196.36) -- (489,196.36) -- cycle ;
%Curve Lines [id:da691862389693042] 
\draw [line width=0.75]    (590.8,116.16) .. controls (573.16,147.52) and (568.97,116.46) .. (549.04,139.67) ;
\draw [shift={(547.8,141.16)}, rotate = 308.93] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-4.9) .. controls (6.95,-2.3) and (3.31,-0.67) .. (0,0) .. controls (3.31,0.67) and (6.95,2.3) .. (10.93,4.9)   ;
%Shape: Rectangle [id:dp29784833864235405] 
\draw  [color={rgb, 255:red, 95; green, 19; blue, 254 }  ,draw opacity=0.23 ][fill={rgb, 255:red, 95; green, 19; blue, 254 }  ,fill opacity=0.23 ] (120.8,155.16) -- (260.8,155.16) -- (260.8,216.36) -- (120.8,216.36) -- cycle ;
%Straight Lines [id:da014819478856842094] 
\draw [line width=1.5]    (81.8,55.36) -- (260.8,55.36) ;
%Straight Lines [id:da19136676020039034] 
\draw [line width=1.5]    (80.8,115.36) -- (260.8,116.36) ;
%Straight Lines [id:da019274737615810222] 
\draw    (61.8,85.36) -- (89.8,85.36) ;
\draw [shift={(91.8,85.36)}, rotate = 180] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da43759945225025065] 
\draw [line width=1.5]    (260.8,55.36) -- (260.8,116.36) ;
%Shape: Rectangle [id:dp8414125012045715] 
\draw  [color={rgb, 255:red, 95; green, 19; blue, 254 }  ,draw opacity=0.23 ][fill={rgb, 255:red, 95; green, 19; blue, 254 }  ,fill opacity=0.23 ] (180.8,55.16) -- (260.8,55.16) -- (260.8,116.36) -- (180.8,116.36) -- cycle ;

% Text Node
\draw (8,176) node [anchor=north west][inner sep=0.75pt]   [align=left] {$\displaystyle A_{2}( t)$};
% Text Node
\draw (7,76) node [anchor=north west][inner sep=0.75pt]   [align=left] {$\displaystyle A_{1}( t)$};
% Text Node
\draw (206,12) node [anchor=north west][inner sep=0.75pt]   [align=left] {$\displaystyle Q_{1}( t)$};
% Text Node
\draw (167,241) node [anchor=north west][inner sep=0.75pt]   [align=left] {$\displaystyle Q_{2}( t)$};
% Text Node
\draw (361,100.4) node [anchor=north west][inner sep=0.75pt]    {$\mathbf{D}( t)$};
% Text Node
\draw (457,65.4) node [anchor=north west][inner sep=0.75pt]  [font=\large]  {$\lambda _{2}$};
% Text Node
\draw (623,196.4) node [anchor=north west][inner sep=0.75pt]  [font=\large]  {$\lambda _{1}$};
% Text Node
\draw (567,94.4) node [anchor=north west][inner sep=0.75pt]  [font=\normalsize]  {$\lambda _{1} +\lambda _{2} =1$};


\end{tikzpicture}

% \begin{tikzpicture}[x=0.5pt,y=0.5pt,yscale=-1,xscale=1]
% %uncomment if require: \path (0,240); %set diagram left start at 0, and has height of 240

% %Straight Lines [id:da09715700995858345] 
% \draw    (85.8,140.36) -- (264.8,139.36) ;
% %Straight Lines [id:da8887479227991981] 
% \draw    (85.8,198.36) -- (265.8,199.36) ;
% %Straight Lines [id:da8614120669050047] 
% \draw    (264.8,139.36) -- (265.8,199.36) ;
% %Straight Lines [id:da6217209993953612] 
% \draw    (54.8,169.36) -- (82.8,169.36) ;
% \draw [shift={(84.8,169.36)}, rotate = 180] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
% %Straight Lines [id:da4398173253440574] 
% \draw    (84.8,40.36) -- (263.8,39.36) ;
% %Straight Lines [id:da5015891688166809] 
% \draw    (84.8,98.36) -- (264.8,99.36) ;
% %Straight Lines [id:da875509031522369] 
% \draw    (263.8,39.36) -- (264.8,99.36) ;
% %Straight Lines [id:da6528587077790915] 
% \draw    (53.8,69.36) -- (81.8,69.36) ;
% \draw [shift={(83.8,69.36)}, rotate = 180] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
% %Rounded Rect [id:dp4517176185326244] 
% \draw  [color={rgb, 255:red, 81; green, 74; blue, 226 }  ,draw opacity=1 ][fill={rgb, 255:red, 74; green, 144; blue, 226 }  ,fill opacity=1 ] (156.8,53.67) .. controls (156.8,47.78) and (161.58,43) .. (167.47,43) -- (250.33,43) .. controls (256.22,43) and (261,47.78) .. (261,53.67) -- (261,85.69) .. controls (261,91.58) and (256.22,96.36) .. (250.33,96.36) -- (167.47,96.36) .. controls (161.58,96.36) and (156.8,91.58) .. (156.8,85.69) -- cycle ;
% %Rounded Rect [id:dp225981923335425] 
% \draw  [color={rgb, 255:red, 81; green, 74; blue, 226 }  ,draw opacity=1 ][fill={rgb, 255:red, 74; green, 144; blue, 226 }  ,fill opacity=1 ] (105.8,153.67) .. controls (105.8,147.78) and (110.58,143) .. (116.47,143) -- (252.33,143) .. controls (258.22,143) and (263,147.78) .. (263,153.67) -- (263,185.69) .. controls (263,191.58) and (258.22,196.36) .. (252.33,196.36) -- (116.47,196.36) .. controls (110.58,196.36) and (105.8,191.58) .. (105.8,185.69) -- cycle ;
% %Straight Lines [id:da37671038244024846] 
% \draw    (156,29) -- (260.8,29) ;
% \draw [shift={(263.8,29)}, rotate = 180] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (8.93,-4.29) -- (0,0) -- (8.93,4.29) -- cycle    ;
% \draw [shift={(153,29)}, rotate = 0] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (8.93,-4.29) -- (0,0) -- (8.93,4.29) -- cycle    ;
% %Straight Lines [id:da0678614898035077] 
% \draw    (111.8,209) -- (263.8,209) ;
% \draw [shift={(266.8,209)}, rotate = 180] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (8.93,-4.29) -- (0,0) -- (8.93,4.29) -- cycle    ;
% \draw [shift={(108.8,209)}, rotate = 0] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (8.93,-4.29) -- (0,0) -- (8.93,4.29) -- cycle    ;
% %Shape: Circle [id:dp028275738414681006] 
% \draw  [fill={rgb, 255:red, 155; green, 155; blue, 155 }  ,fill opacity=0.67 ] (365,126.18) .. controls (365,118) and (371.63,111.36) .. (379.82,111.36) .. controls (388,111.36) and (394.64,118) .. (394.64,126.18) .. controls (394.64,134.37) and (388,141) .. (379.82,141) .. controls (371.63,141) and (365,134.37) .. (365,126.18) -- cycle ;
% %Curve Lines [id:da7202837492936005] 
% \draw    (343.8,61.36) .. controls (279.45,106.9) and (302.33,157.34) .. (342.58,188.43) ;
% \draw [shift={(343.8,189.36)}, rotate = 217.09] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
% %Straight Lines [id:da4678251099443136] 
% \draw    (365,126.18) -- (288.45,73.5) ;
% \draw [shift={(286.8,72.36)}, rotate = 394.53999999999996] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
% %Shape: Axis 2D [id:dp8494447421977243] 
% \draw [line width=1.5]  (461,179.73) -- (637.8,179.73)(478.68,48) -- (478.68,194.36) (630.8,174.73) -- (637.8,179.73) -- (630.8,184.73) (473.68,55) -- (478.68,48) -- (483.68,55)  ;
% %Shape: Right Triangle [id:dp441461564376495] 
% \draw  [fill={rgb, 255:red, 74; green, 120; blue, 226 }  ,fill opacity=0.6 ] (478,79) -- (599.8,180.36) -- (478,180.36) -- cycle ;
% %Curve Lines [id:da691862389693042] 
% \draw [line width=0.75]    (579.8,100.16) .. controls (562.16,131.52) and (557.97,100.46) .. (538.04,123.67) ;
% \draw [shift={(536.8,125.16)}, rotate = 308.93] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-4.9) .. controls (6.95,-2.3) and (3.31,-0.67) .. (0,0) .. controls (3.31,0.67) and (6.95,2.3) .. (10.93,4.9)   ;

% % Text Node
% \draw (8,160) node [anchor=north west][inner sep=0.75pt]   [align=left] {$\displaystyle A_{2}( t)$};
% % Text Node
% \draw (7,60) node [anchor=north west][inner sep=0.75pt]   [align=left] {$\displaystyle A_{1}( t)$};
% % Text Node
% \draw (186,5) node [anchor=north west][inner sep=0.75pt]   [align=left] {$\displaystyle Q_{1}( t)$};
% % Text Node
% \draw (169,213) node [anchor=north west][inner sep=0.75pt]   [align=left] {$\displaystyle Q_{2}( t)$};
% % Text Node
% \draw (361,88.4) node [anchor=north west][inner sep=0.75pt]    {$\mathbf{D}( t)$};
% % Text Node
% \draw (446,49.4) node [anchor=north west][inner sep=0.75pt]  [font=\large]  {$\lambda _{2}$};
% % Text Node
% \draw (612,180.4) node [anchor=north west][inner sep=0.75pt]  [font=\large]  {$\lambda _{1}$};
% % Text Node
% \draw    (526,68) -- (635,68) -- (635,99) -- (526,99) -- cycle  ;
% \draw (529,72.4) node [anchor=north west][inner sep=0.75pt]  [font=\large]  {$\lambda _{1} +\lambda _{2} \leq 1$};
% % Text Node
% \draw (461,175.4) node [anchor=north west][inner sep=0.75pt]  [font=\Large]  {$o$};


%\end{tikzpicture}
}

==> figures/queueing_system_only.tex <==


\tikzset{every picture/.style={line width=0.75pt}} %set default line width to 0.75pt        

% SYNTAX: \resizebox{width}{height}
\resizebox{5.50cm}{3.5cm}{

\begin{tikzpicture}[x=0.5pt,y=0.5pt,yscale=-1,xscale=1]
%uncomment if require: \path (0,273); %set diagram left start at 0, and has height of 273

%Straight Lines [id:da09715700995858345] 
\draw [line width=1.5]    (91.11,161.23) -- (292.11,161.23) ;
%Straight Lines [id:da8887479227991981] 
\draw [line width=1.5]    (89.99,227.37) -- (292.11,228.47) ;
%Straight Lines [id:da6217209993953612] 
\draw    (68.66,194.3) -- (100.34,194.3) ;
\draw [shift={(102.34,194.3)}, rotate = 180] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da875509031522369] 
\draw [line width=1.5]    (292.11,161.23) -- (292.11,228.47) ;
%Straight Lines [id:da37671038244024846] 
\draw    (201.01,39.58) -- (289.11,39.58) ;
\draw [shift={(292.11,39.58)}, rotate = 180] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (8.93,-4.29) -- (0,0) -- (8.93,4.29) -- cycle    ;
\draw [shift={(198.01,39.58)}, rotate = 0] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (8.93,-4.29) -- (0,0) -- (8.93,4.29) -- cycle    ;
%Straight Lines [id:da0678614898035077] 
\draw    (136.78,237.99) -- (289.11,237.99) ;
\draw [shift={(292.11,237.99)}, rotate = 180] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (8.93,-4.29) -- (0,0) -- (8.93,4.29) -- cycle    ;
\draw [shift={(133.78,237.99)}, rotate = 0] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (8.93,-4.29) -- (0,0) -- (8.93,4.29) -- cycle    ;
%Shape: Ellipse [id:dp028275738414681006] 
\draw  [fill={rgb, 255:red, 155; green, 155; blue, 155 }  ,fill opacity=0.67 ] (409.11,146.7) .. controls (409.11,137.68) and (416.56,130.37) .. (425.75,130.37) .. controls (434.94,130.37) and (442.39,137.68) .. (442.39,146.7) .. controls (442.39,155.72) and (434.94,163.04) .. (425.75,163.04) .. controls (416.56,163.04) and (409.11,155.72) .. (409.11,146.7) -- cycle ;
%Curve Lines [id:da7202837492936005] 
\draw    (385.31,75.25) .. controls (313.05,125.45) and (338.74,181.05) .. (383.93,215.31) ;
\draw [shift={(385.31,216.35)}, rotate = 216.57999999999998] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da4678251099443136] 
\draw    (409.11,146.7) -- (322.96,88.5) ;
\draw [shift={(321.3,87.38)}, rotate = 394.03999999999996] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Shape: Rectangle [id:dp29784833864235405] 
\draw  [color={rgb, 255:red, 95; green, 19; blue, 254 }  ,draw opacity=0.23 ][fill={rgb, 255:red, 95; green, 19; blue, 254 }  ,fill opacity=0.23 ] (139.8,161.01) -- (292.11,161.01) -- (292.11,228.47) -- (139.8,228.47) -- cycle ;
%Straight Lines [id:da014819478856842094] 
\draw [line width=1.5]    (91.11,51) -- (292.11,51) ;
%Straight Lines [id:da19136676020039034] 
\draw [line width=1.5]    (89.99,117.14) -- (292.11,118.24) ;
%Straight Lines [id:da019274737615810222] 
\draw    (68.66,84.07) -- (100.34,84.07) ;
\draw [shift={(102.34,84.07)}, rotate = 180] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da43759945225025065] 
\draw [line width=1.5]    (292.11,51) -- (292.11,118.24) ;
%Shape: Rectangle [id:dp8414125012045715] 
\draw  [color={rgb, 255:red, 95; green, 19; blue, 254 }  ,draw opacity=0.23 ][fill={rgb, 255:red, 95; green, 19; blue, 254 }  ,fill opacity=0.23 ] (209.8,50.78) -- (292.11,50.78) -- (292.11,118.24) -- (209.8,118.24) -- cycle ;

% Text Node
\draw (10.64,184.95) node [anchor=north west][inner sep=0.75pt]   [align=left] {$\displaystyle A_{2}( t)$};
% Text Node
\draw (9.52,74.72) node [anchor=north west][inner sep=0.75pt]   [align=left] {$\displaystyle A_{1}( t)$};
% Text Node
\draw (233.03,4.18) node [anchor=north west][inner sep=0.75pt]   [align=left] {$\displaystyle Q_{1}( t)$};
% Text Node
\draw (195.98,249.99) node [anchor=north west][inner sep=0.75pt]   [align=left] {$\displaystyle Q_{2}( t)$};
% Text Node
\draw (406.65,101.42) node [anchor=north west][inner sep=0.75pt]    {$\mathbf{D}( t)$};


\end{tikzpicture}
}
